Personalised Federated Learning On Heterogeneous Feature Spaces

Most personalised federated learning (FL) approaches assume that raw data of all clients are defined in a common subspace i.e. all clients store their data according to the same schema. For real-world applications, this assumption is restrictive as clients, having their own systems to collect and then store data, may use heterogeneous data representations. We aim at filling this gap. To this end, we propose a general framework coined FLIC that maps client's data onto a common feature space via local embedding functions. The common feature space is learnt in a federated manner using Wasserstein barycenters while the local embedding functions are trained on each client via distribution alignment. We integrate this distribution alignement mechanism into a federated learning approach and provide the algorithmics of FLIC. We compare its performances against FL benchmarks involving heterogeneous input features spaces. In addition, we provide theoretical insights supporting the relevance of our methodology.

==> macros.tex <==
\definecolor{darkgreen}{RGB}{0,128,0}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{darkblue}{RGB}{0,0,139}
\renewcommand{\algorithmiccomment}[1]{ \textcolor{darkgreen}{// \texttt{#1}}}%\verb|\textcolor{green}{#1}|}

%% Commands %%
% \newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\normTV}[1]{\left\|#1\right\|_{\mathrm{TV}}}
% \newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\tbtheta}{\tilde{x}}
% \newcommand{\bz}{\B{z}}
\newcommand{\Zrm}{\mathrm{Z}}
% \newcommand{\bx}{\B{x}}
% \newcommand{\by}{\B{y}}
% \newcommand{\dd}{\mathrm{d}}
% \newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rn}{\mathbb{R}^n}
% \newcommand{\grad}{\nabla}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\bthetastar}{\boldsymbol{x^{\star}}}
\newcommand{\subscript}[2]{$#1 _ #2$}
% \newcommand{\oh}{\operatorname{\mathrm{o}}}
% \newcommand{\Oh}{\operatorname{\mathrm{O}}}
% \newcommand{\1}{\mathds{1}}
\newcommand{\X}{\mathscr{X}}
% \newcommand{\R}{\mathbb{R}}
 \newcommand{\PVar}{\operatorname{Var}}
  \newcommand{\var}[1]{\operatorname{Var}\parenthese{#1}}
    \newcommand{\varLigne}[1]{\operatorname{Var}\parentheseLigne{#1}}


% Parenthèses, Crochets et Accolades
% \newcommand{\pr}[1]{\left({#1}\right)}
% \newcommand{\prn}[1]{({#1})}
% \newcommand{\prbig}[1]{\big({#1}\big)}
% \newcommand{\prBig}[1]{\Big({#1}\Big)}
% \newcommand{\prbigg}[1]{\bigg({#1}\bigg)}
% \newcommand{\prBigg}[1]{\Bigg({#1}\Bigg)}
% \newcommand{\br}[1]{\left[{#1}\right]}
% \newcommand{\brn}[1]{[{#1}]}
% \newcommand{\brbig}[1]{\big[{#1}\big]}
% \newcommand{\brBig}[1]{\Big[{#1}\Big]}
% \newcommand{\brbigg}[1]{\bigg[{#1}\bigg]}
% \newcommand{\brBigg}[1]{\Bigg[{#1}\Bigg]}
% \newcommand{\ac}[1]{\left\{{#1}\right\}}
% \newcommand{\acn}[1]{\{{#1}\}}
% \newcommand{\acbig}[1]{\big\{{#1}\big\}}
% \newcommand{\acBig}[1]{\Big\{{#1}\Big\}}
% \newcommand{\acbigg}[1]{\bigg\{{#1}\bigg\}}
% \newcommand{\acBigg}[1]{\Bigg\{{#1}\Bigg\}}
% \newcommand{\normn}[1]{\|{#1}\|}
% \newcommand{\normbig}[1]{\big\|{#1}\big\|}
% \newcommand{\normBig}[1]{\Big\|{#1}\Big\|}
% \newcommand{\normbigg}[1]{\bigg\|{#1}\bigg\|}

% % Quand on râle sur les fractions :
% \newcommand{\nofrac}[2]{{#1}/{#2}}
% % Quand on râle sur les racines carrées :
% \newcommand{\nosqrt}[1]{{#1}^{\half}}

% % Pour discuter entre nous :
% \newcommand{\vp}[1]{\textcolor{blue}{\small\slshape [VP: #1]}}
% % Pour mettre en évidence les modifications :
% \newcommand{\changed}[1]{\textcolor{red}{#1}}
% % Pour les espaces
% \def\eqsp{\;}

% \renewcommandx{\iint}[2][1=]{\ifthenelse{\equal{#1}{}}{[#2]}{[#1:#2]}}

%%%%%%%%%%%%%%%
%% mathbf
\def\bfn{\mathbf{n}}
\def\bfbeta{\boldsymbol{\beta}}
\def\bfx{\mathbf{x}}
\def\xbf{\mathbf{x}}


%%% mathsf
\def\msi{\mathsf{I}}
% \def\msa{\mathsf{A}}
\def\tmsa{\tilde{\msa}}
\def\msd{\mathsf{D}}
\def\msz{\mathsf{Z}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}}
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{o}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
% \def\msx{\mathsf{X}}
% \def\msy{\mathsf{Y}}



%% mathcal
\def\mca{\mathcal{A}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcb{\mathcal{B}}
%\newcommand{\mcb}[1]{\mathcal{B}(#1)}
\def\mcc{\mathcal{C}}
% \def\mcy{\mathcal{Y}}
% \def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}
\def\mct{\mathcal{T}}

%% mathbb

\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}


%%%% mathrm

\def\rmb{\mathrm{b}}
\def\mrb{\mathrm{b}}
\def\mrl{\mathrm{L}}
\def\rml{\mathrm{L}}
\def\rmd{\mathrm{d}}
\def\rmZ{\mathrm{Z}}
\def\mrd{\mathrm{d}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrc{\mathrm{C}}
\def\mrcc{\mathrm{c}}
\def\rmc{\mathrm{C}}
\def\rmC{\mathrm{C}}
\def\rmcc{\mathrm{c}}
\def\rma{\mathrm{a}}
\def\mra{\mathrm{a}}
\def\rmF{\mathrm{F}}
\def\rmE{\mathrm{E}}


\newcommand{\cco}{\llbracket}
\newcommand{\ccf}{\rrbracket}
\newcommand{\po}{\left(}
\newcommand{\pf}{\right)}
\newcommand{\co}{\left[}
\newcommand{\cf}{\right]}
\newcommand{\D}{\mathcal D}
\newcommand{\A}{\mathcal A}
% \newcommand{\M}{\mathcal M}
\newcommand{\na}{\nabla}
\newcommand{\loiy}{\mu_{\mathrm{v}}}
\newcommand{\rem}[1]{\textcolor{red}{(#1)}}



\def\MeasFspace{\mathbb{M}}
\def\xstar{x^\star}
\def\Tr{\operatorname{T}}
\def\trace{\operatorname{Tr}}
% \newcommandx{\functionspace}[2][1=+]{\mathbb{F}_{#1}(#2)}
%% argmin, argmax
\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argsort}{\operatorname*{arg\,sort}}
% \newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\estimateur}[1]{\hat{\pi}_n^N(#1)}
\def\RichR{\operatorname{R}}
\def\piR{\hat{\pi}^{\RichR}}
\def\estimatorRR{\piR}
% \newcommandx{\VarDeux}[3][3=]{\operatorname{Var}^{#3}_{#1}\left\{#2 \right\}}
\newcommand{\VarDeuxLigne}[2]{\operatorname{Var}_{#1}\{#2 \}}
\newcommand{\gramm}{\operatorname{Gramm}}
% \newcommand{\2}[1]{\mathbbm{1}_{\{#1\}}}




\newcommand{\LeftEqNo}{\let\veqno\@@leqno}

\newcommand{\lambdast}{\lambda^{s \rightarrow t}}
\newcommand{\etast}{\eta^{s \rightarrow t}}
\newcommand{\mst}{m^{s \rightarrow t}}
\newcommand{\mun}{m^{1 \rightarrow 2}}
\newcommand{\mdeux}{m^{2 \rightarrow 1}}
\newcommand{\lambdaun}{\lambda^{2 \rightarrow 1}}
\newcommand{\etaun}{\eta^{2 \rightarrow 1}}
\newcommand{\lambdadeux}{\lambda^{1 \rightarrow 2}}
\newcommand{\etadeux}{\eta^{1 \rightarrow 2}}
\newcommand{\mnun}{m^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\etanun}{\eta^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\lambdanun}{\lambda^{n+1 \rightarrow \pi(n+1)}}
\newcommand{\xpinun}{x_{\pi(n+1)}}
\newcommand{\xnun}{x_{n+1}}
\newcommand{\mpinun}{m^{\pi(n+1) \rightarrow n+1}}
\newcommand{\etapinun}{\eta^{\pi(n+1) \rightarrow n+1}}
\newcommand{\lambdapinun}{\lambda^{\pi(n+1) \rightarrow n+1}}
\newcommand{\pinun}{\pi(n+1)}
\newcommand{\vois}{\mathcal{N}}
\newcommand{\mpii}{m^{i \rightarrow \pi(n+1)}}
\newcommand{\etapii}{\eta^{i \rightarrow \pi(n+1)}}
\newcommand{\lambdapii}{\lambda^{i \rightarrow \pi(n+1)}}
\newcommand{\alphahat}{\widehat{\alpha}}
\newcommand{\betahat}{\widehat{\beta}}
\newcommand{\tildegamma}{\widetilde{\gamma}}
\newcommand{\tildeP}{\widetilde{P}}

\newcommand{\myeqref}[1]{Eq.~\eqref{#1}}



%%%% Floating Points Notation

\newcommand{\fpround}[1]{\lfloor #1 \rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\ceilLigne}[1]{\lceil #1 \rceil}
\newcommand{\floorLigne}[1]{\lfloor #1 \rfloor}
\newcommand{\inv}[1]{\frac{1}{#1}}


%voc
\newcommand{\pth}{\ensuremath{p^{\text{th}}}}
\newcommand{\qth}{\ensuremath{q^{\text{th}}}}
\newcommand{\nth}{\ensuremath{n^{\text{th}}}}

%order
\newcommand{\ord}{\ensuremath{\operatorname{ord}}}
\newcommand{\rad}{\ensuremath{\operatorname{rad}}}



% Sets
% \newcommand{\N}{\ensuremath{\mathbb{N}}}
% \newcommand{\Q}{\ensuremath{\mathbb{Q}}}
% \newcommand{\C}{\ensuremath{\mathbb{C}}}

%\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\primes}{\ensuremath{\mathcal P}}

\newcommand{\sfi}{\ensuremath{\mathcal{S}\!\mathcal{F}}}
\newcommand{\sfibt}{\ensuremath{\mathcal{S}\!\mathcal{F}'}}

\newcommand{\reghat}{\widehat{R}}

\newcommand{\reghatn}{\widehat{R}_n}

\newcommand{\arm}{\mathcal{A}}

\newcommand{\mX}{\widehat{X}}
\newcommand{\PE}{\mathbb{E}}
\newcommand{\Ft}{\mathcal{F}}

\newcommand{\Sy}{\mathbf{S}}

\newcommand{\Kfrac}{\mathscr{K}}

% Operands
\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
% \newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
% \newcommandx{\VnormEq}[2][1=V]{\left\| #2 \right\|_{#1}}
\newcommand{\normLigne}[1]{\Vert #1 \Vert}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLignebig}[1]{\big(#1 \big)}
\newcommand{\parentheseLigneBig}[1]{\Big(#1 \Big)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }

% \newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}
\newcommand{\psLigne}[2]{\langle#1,#2 \rangle}
\newcommand{\psmu}[2]{\left\langle#1,#2 \right\rangle_{\mu}}
\newcommand{\psmuLigne}[2]{\langle#1,#2 \rangle_{\mu}}

\newcommand{\eqdef}{\overset{\text{\tiny def}} =}
\newcommand{\defeq}{\overset{\text{\tiny def}} =}

% Relations
\newcommand{\divid}{\mid}
\newcommand{\ndivide}{\nmid}

% Proba
% \newcommand{\proba}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\probaCond}[2]{\mathbb{P}\left( \left. #1  \middle\vert #2 \right.\right)}
\newcommand{\probaLigne}[1]{\mathbb{P}( #1 )}
% \newcommandx\probaMarkovTilde[2][2=]
% {\ifthenelse{\equal{#2}{}}{{\widetilde{\mathbb{P}}_{#1}}}{\widetilde{\mathbb{P}}_{#1}\left[ #2\right]}}
\newcommand{\probaMarkov}[2]{\mathbb{P}_{#1}\left( #2\right)}
\newcommand{\expe}[1]{\PE \left[ #1 \right]}
\newcommand{\expeExpo}[2]{\PE^{#1} \left[ #2 \right]}
\newcommand{\expeLigne}[1]{\PE [ #1 ]}
\newcommand{\expeLine}[1]{\PE [ #1 ]}
\newcommand{\expeMarkov}[2]{\PE_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovLigne}[2]{\PE_{#1} [ #2 ]}
\newcommand{\expeMarkovExpo}[3]{\PE_{#1}^{#2} \left[ #3 \right]}
\newcommand{\probaMarkovTildeDeux}[2]{\widetilde{\mathbb{P}}_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovTilde}[2]{\widetilde{\PE}_{#1} \left[ #2 \right]}

% Landau notation (big O)
\newcommand{\bigO}{\ensuremath{\mathcal{O}}}
\newcommand{\softO}{\Tilde{\ensuremath{\mathcal{O}}}}

% Environments

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%\renewenvironment{proof}[1][{\textit{Proof:}}]{\begin{trivlist} \item[\em{\hskip \labelsep #1}]}{\ensuremath{\qed} \end{trivlist}}

%fleche limite
\newcommand{\flecheLimite}{\underset{n\to+\infty}{\longrightarrow}}
\newcommand{\flecheLimiteOption}[2]{\underset{#1\to#2}{\longrightarrow}}
\newcommand{\flecheLimiteHaut}{\overset{n\to+\infty}{\longrightarrow}}


%notation infini
\newcommand{\plusinfty}{+\infty}

%notation egale
\newcommand{\egale}[1]{\ensuremath{\underset{#1}{=}}}

%plusieurs ligne indice
%\sum\limits_{\substack{i=0 \\ i \neq i_0}}^{n}{A_

\newcommand{\hilbert}{\mathcal{H}}


\def\ie{\textit{i.e. }}
\def\cadlag{càdlàg}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}

\def\primr{f_r}
\def\primrO{f_{r_0}}

\newcommand{\indi}[1]{\1_{#1}}
% \newcommandx{\weight}[2][2=n]{\omega_{#1,#2}^N}
\newcommand{\loi}{\mathcal{L}}
\newcommand{\boule}[2]{\operatorname{B}(#1,#2)}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\boulefermee}[2]{\overline{B}(#1,#2)}
\newcommand{\diameter}{\operatorname{diam}}
\newcommand{\deta}{d_{\eta}}

\def\TV{\mathrm{TV}}

\newcommand{\alain}[1]{\todo[color=blue!20]{{\bf AD:} #1}}
\newcommand{\maxime}[1]{\todo[color=blue!20]{{\bf MV:} #1}}
\newcommand{\vincent}[1]{\todo[color=blue!20]{{\bf VP:} #1}}
\newcommand{\aymeric}[1]{\todo[color=blue!20]{{\bf AyD:} #1}}
\newcommand{\eric}[1]{\todo[color=red!20]{{\bf EM:} #1}}

\newcommand{\tcr}[1]{\textcolor{red}{#1}}



\def\as{\ensuremath{\text{a.s.}}}
\def\dist{\operatorname{dist}}

\newcommandx\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{( #1_{#2})}}{\ensuremath{( #1_{#2})_{ #2 \in #3}}}}

\newcommandx\sequencet[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{( #1_{#2})}}{\ensuremath{( #1_{#2})_{ #2 \geq #3}}}}
% \newcommandx\sequence[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}
% \newcommandx\sequenceD[3][2=,3=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{( #1)_{ #2 \in #3} }}}

% \newcommandx{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}
% \newcommandx\sequenceDouble[4][3=,4=]
% {\ifthenelse{\equal{#3}{}}{\ensuremath{\{ (#1_{#3},#2_{#3}) \}}}{\ensuremath{\{  (#1_{#3},#2_{#3}), \eqsp #3 \in #4 \}}}}
% \newcommandx{\sequencenDouble}[3][3=n\in\N]{\ensuremath{\{ (#1_{n},#2_{n}), \eqsp #3 \}}}

\newcommand{\wrt}{w.r.t.}
\newcommand{\Withoutlog}{w.l.o.g.}
\def\iid{\text{i.i.d.}}
\def\ifof{if and only if}
\def\eg{e.g.}

% \newcommand{\note}[1]{{\textbf{\color{red}#1}}}

\newcommand{\opnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\normLip}[1]{\left\Vert #1 \right\Vert_{\text{Lip}}}
\newcommand{\normLipLoc}[1]{\left\Vert #1 \right\Vert_{\text{LipLoc}}}

\def\Lip{\operatorname{Lip}}
\def\generator{\mathcal{A}}
\def\generatorsp{\generator^{\sphere^d}}
\def\generatorr{\generator^{\rset^d}}

\def\momentNoise{\mathrm{m}}
\def\bfe{\mathbf{e}}

\def\bfv{\mathbf{v}}
\def\ebf{\mathbf{e}}
\def\vbf{\mathbf{v}}

\def\Id{\operatorname{Id}}

\def\tildetheta{\tilde{\theta}}

\def\calC{\mathcal{C}}

% \newcommandx{\CPE}[3][1=]{{\mathbb E}_{#1}\left[#2 \left \vert #3 \right. \right]} %%%% esperance conditionnelle
% \newcommandx{\CPVar}[3][1=]{\mathrm{Var}^{#3}_{#1}\left\{ #2 \right\}}
% \newcommand{\CPP}[3][]
% {\ifthenelse{\equal{#1}{}}{{\mathbb P}\left(\left. #2 \, \right| #3 \right)}{{\mathbb P}_{#1}\left(\left. #2 \, \right | #3 \right)}}

\def\Ascr{\mathscr{A}}
\def\Dscr{\mathscr{D}}
\def\scrD{\mathscr{D}}
\def\scrA{\mathscr{A}}
\def\scrB{\mathscr{B}}
\def\scrC{\mathscr{C}}
\def\scrT{\mathscr{T}}
\def\scrF{\mathscr{F}}

\def\barL{\bar{L}}

\def\YL{\mathbf{Y}}
\def\XEM{X}
\def\steps{\gamma}
\def\measSet{\mathbb{M}}

\newcommand\Ent[2]{\mathrm{Ent}_{#1}\left(#2\right)}
% \newcommandx{\osc}[2][1=]{\mathrm{osc}_{#1}(#2)}

% \def\Ybar{\bar{Y}}
\def\Id{\operatorname{Id}}
\def\IdM{\operatorname{I}_d}
\newcommand\EntDeux[2]{\Ent_{#1}\left[#2 \right]}
\def\Ltwo{\mathrm{L}^2}
\def\Lone{\mathrm{L}^1}
\newcommand\densityPi[1]{\frac{\rmd #1}{\rmd \pi}}
\newcommand\densityPiLigne[1]{\rmd #1 /\rmd \pi}
\newcommand\density[2]{\frac{\rmd #1}{\rmd #2}}
\newcommand\densityLigne[2]{\rmd #1/\rmd #2}

\def\V{V}
\def\VD{V}
\def\Vsp{V^{\sphere^d}_{\b,\beta}}
\def\Vr{V^{\rset^d}_{\b,\c,\beta}}

\def\Prset{P^{\rset^d}}
\def\Psphere{P^{\sphere^d}}

\def\n{\mathrm{n}}
\def\Vpsi{\psi}
\def\Vkappa{\kappa}
\def\Vkappat{\tilde{\kappa}}
\def\Vchi{\chi}
\def\Vchit{\tilde{\chi}}
\def\Vphi{\phi}
\def\Vrho{\rho}
\def\psiV{\Vpsi}
\def\rhoV{\Vrho}
\def\phiV{\Vphi}
\def\fV{f}
\def\Vf{\fV}
\def\kappaVt{\tilde{\Vkappa}}
\def\kappaV{\Vkappa}
\def\chiV{\Vchi}
\def\chiVt{\Vchit}


\def\a{a}
\def\b{b}
\def\c{c}
\def\e{e}
\def\rU{\mathrm{r}}

\def\domain{\mathrm{D}}

\def\martfg{M^{f,g}}
\newcommand\Ddir[1]{D_{#1}}
\newcommand\maxplus[1]{\parenthese{#1}_+}
\def\Refl{\mathrm{R}}
\def\phibf{\pmb{\phi}}
\def\Gammabf{\mathbf{\Gamma}}

\def\transpose{\operatorname{T}}
\def\v{v}
\def\w{w}
\def\y{y}
\def\z{z}
%%%% bar

\def\bU{\bar{U}}
\def\Ub{\bU}
\def\lambdab{\bar{\lambda}}
\def\blambdab{\bar{\lambda}}
\def\bv{\bar{v}}
\def\vb{\bv}
\def\yb{\bar{y}}
%\def\by{\yb}
\def\Xb{\bar{X}}
%\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\taub{\bar{\tau}}

\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bF{\bar{F}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}

\def\pib{\bar{\pi}}
\def\bpi{\pib}

\def\S{S}

%%%% normal

\def\nE{E}
\def\nF{F}


%%%% tilde

\def\tF{\tilde{F}}
\def\tmsk{\tilde{\msk}}
\def\tW{\tilde{W}}
\def\tvarsigma{\tilde{\varsigma}}
\def\tv{\tilde{v}}
\def\vt{\tv}
\def\yt{\tilde{y}}
\def\ty{\yt}
\def\Mt{\tilde{M}}
\def\tM{\Mt}

\def\tx{\tilde{x}}
\def\xt{\tx}
\def\tbfx{\tilde{\bfx}}
\def\txbf{\tbfx}
\def\Xt{\tilde{X}}
\def\Yt{\tilde{Y}}
\def\Gt{\tilde{G}}
\def\Et{\tilde{E}}
\def\Tt{\tilde{T}}
\def\St{\tilde{S}}
\def\taut{\tilde{\tau}}

\def\tX{\tilde{X}}
\def\tY{\tilde{Y}}
\def\tG{\tilde{G}}
\def\tE{\tilde{E}}
\def\tT{\tilde{T}}
\def\tS{\tilde{S}}
\def\ttau{\tilde{\tau}}


\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Gb{\bar{G}}
\def\Eb{\bar{E}}
\def\Tb{\bar{T}}
\def\Sb{\bar{S}}
\def\taub{\bar{\tau}}
\def\Hb{\bar{H}}
\def\Nb{\bar{N}}


\def\bX{\bar{X}}
\def\bY{\bar{Y}}
\def\bG{\bar{G}}
\def\bE{\bar{E}}
\def\bT{\bar{T}}
\def\btau{\bar{\tau}}
\def\bS{\bar{S}}
\def\bSigma{\bar{\Sigma}}
\def\bH{\bar{H}}
\def\bN{\bar{N}}

%%%%%%%%

\def\mgU{\mathrm{m}_{\nabla U}}
\def\MintDrift{I}
\def\CU{C_U}
\def\RU{R_1}
\def\RV{R}
\def\Reps{R_{\epsilon}}
\def\Resp{\Reps}
\def\veps{\varepsilon}
\def\sphere{\mss}

\def\nablaUt{\overline{\nabla U}}
\def\measureSphere{\nu^d}

\def\etaU{\eta}
\def\epsilonU{\epsilon}

\def\Jac{\operatorname{Jac}}
\def\jac{\operatorname{Jac}}
\def\sign{\operatorname{sign}}
\def\rate{\lambda_{\mathrm{r}}}
\def\sigmaS{\sigma^2}

\def\rmD{\mathrm{D}}%%rmd déjà pris
\def\mrd{\mathrm{D}}
\def\mrc{\mathrm{C}}

\def\diag{\Delta_{\rset^d}}

\def\lyap{V}
\def\supp{\mathrm{supp}}
\def\tpi{\tilde{\pi}}

\newcommand\coupling[2]{\Gamma(\mu,\nu)}
\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}
\newcommand\adh[1]{\overline{#1}}
\newcommand{\fracm}[2]{\left. #1 \middle / #2 \right.}
\newcommand{\comp}{\mathrm{c}}
\newcommand{\fraca}[2]{(#1/#2)}
% \newcommand{\half}{{\nicefrac{1}{2}}}
% \newcommandx{\wasserstein}[2][1=2]{\ifthenelse{\equal{#1}{}}{W}{W_{#1}}}
% \newcommandx{\wassersteinLigne}[3][1=\distance,3=]{\mathbf{W}_{#1}^{#3}(#2)}
% \newcommandx{\wassersteinD}[1][1=\distance]{\mathbf{W}_{#1}}
% \newcommandx{\wassersteinDLigne}[1][1=\distance]{\mathbf{W}_{#1}}

\def\ACb{\mathrm{AC}_{\mathrm{b}}}
\def\opK{\mathrm{K}}

\def\poty{H}
\def\diam{\mathrm{diam}}
\def\talpha{\tilde{\alpha}}
\def\Leb{\mathrm{Leb}}
\newcommand{\iintD}[2]{\{#1,\ldots,#2\}}
\def\interior{\mathrm{int}}
\def\iff{ if and only if }

\def\vareps{\varepsilon}
\def\varespilon{\varepsilon}
\def\si{\text{ if } }
\def\projd{\operatorname{proj}^{\msd}}
\def\projp{\operatorname{proj}^{\msp}}
\def\projz{\operatorname{proj}_{\msz}}
\def\Phibf{\mathbf{\Phi}}

\def\th{\tilde{h}}
\def\thg{\th_{\gamma}}
\def\hg{h_{\gamma}}
\def\bgamma{\bar{\gamma}}
\def\bdelta{\bar{\delta}}
\def\tZ{\tilde{Z}}
\def\tP{\tilde{P}}
\def\tQ{\tilde{Q}}

\def\varphibf{\boldsymbol{\varphi}}
\def\InftyBound{c_\infty}
\def\bfz{\mathbf{z}}
\def\zbf{\bfz}
\def\tbfz{\tilde{\mathbf{z}}}
\def\tzbf{\tbfz}

\def\bfr{\mathbf{r}}
\def\rbf{\bfr}
\def\bfm{\mathbf{m}}
\def\rbm{\bfm}

\def\Ltt{\mathtt{L}}
\def\mtt{\mathtt{m}}
\def\Btt{\mathtt{B}}
\def\Mtt{\mathtt{M}}
\def\tMtt{\tilde{\mathtt{M}}}
\def\bMtt{\bar{\mathtt{M}}}

\def\tR{\tilde{R}}
\def\a{\mathbf{a}}
\def\bpg{\overline{p}_{\sigma^2\gamma}}
\def\tw{\tilde{w}}
\def\rmT{\mathrm{T}}
\def\trmT{\tilde{\rmT}}

\def\deltaInf{\bdelta}
\def\tmu{\tilde{\mu}}

\def\cbf{\mathbf{c}}
\def\tcbf{\tilde{\cbf}}
\def\tpi{\tilde{\pi}}

\def\lyapD{\mathpzc{V}}
\def\LyapD{\mathpzc{V}}
\def\VlyapD{\mathpzc{V}}

\def\lyapDs{\mathpzc{V}^*}
\def\LyapDs{\mathpzc{V}^*}
\def\VlyapDs{\mathpzc{V}^*}

\def\tauginf{\tau_{\gamma}^{\infty}}

\def\constMoment{c}
\def\Wn{W^{(n)}}
\def\Wnbf{\mathbf{W}^{(n)}}

\def\wiener{\mathbb{W}}
\def\wienersigma{\mathcal{W}}
\def\proccano{\mathrm{W}}
\def\canoproc{\proccano}

\def\Wbf{\mathbf{W}}
\def\mubf{\boldsymbol{\mu}}
\def\Wbfn{\Wbf^{(n)}}

\def\thetabf{\btheta}
\def\bftheta{\btheta}
\def\tthetabf{\tbtheta}
\def\tbftheta{\tbtheta}

\def\Abf{\mathbf{A}}
\def\bfA{\mathbf{A}}
\def\bfB{\mathbf{B}}
\def\Bbf{\mathbf{B}}
\def\bfa{\mathbf{a}}
\def\bfgamma{\boldsymbol{\gamma}}
\def\gammabf{\bfgamma}
\def\bfrho{\boldsymbol{\rho}}
\def\rhobf{\boldsymbol{\rho}}
\def\bfN{\boldsymbol{N}}
\def\bbfA{\bar{\bfA}}
\def\bbfB{\bar{\bfB}}
\def\bfOne{\boldsymbol{1}}

% Define the notations of prop3
\def\Idp{\mathbf{I}_p}
\def\Yb{Y}
% \def\Yc{\tilde{Y}}
\def\Ybr{\mathrm{Y}}
\def\Ycr{\tilde{\mathrm{Y}}}
\def\Zb{Z}
\def\Zc{\tilde{Z}}

% \newcommand{\txts}{\textstyle}
\def\loiGauss{\mathrm{N}}
\def\tPi{\tilde{\Pi}}
\def\tildeU{V}


\newcommand{\vp}[1]{\textcolor{blue}{[VP: {#1}]}}  % PineGreen
\newcommand{\auchoix}[1]{\textcolor{cyan}{[auchoix: {#1}]}}  % MidnightBlue
% Pour mettre en évidence les modifications :
\newcommand{\note}[1]{\textcolor{red}{\newline[note: {#1}]\hrule}}

% ---------------------
%\hypersetup{colorlinks = true, urlcolor = blue, bookmarksopen = true}

% On définit les ensembles (plutôt utile en mathématiques...):
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\msa}{\mathsf{A}}
\newcommand{\msx}{\mathsf{X}}
\newcommand{\msy}{\mathsf{Y}}
\newcommand{\mcy}{\mathcal{Y}}
\newcommand{\mcx}{\mathcal{X}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Rd}{\mathbb{R}^{d}}

% On définit des commandes générales
\newcommand{\dd}{\mathrm{d}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\T}{\intercal}
\newcommand{\argmin}{\operatornamewithlimits{\arg\min}}
\newcommand{\oh}{\operatorname{\mathrm{o}}}
\newcommand{\Oh}{\operatorname{\mathrm{O}}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\cov}{\operatorname{cov}}
% Pour les indices :
\newcommand{\half}{1/2}  % \nicefrac{1}{2}
% Quand on râle sur les fractions :
\newcommand{\nofrac}[2]{{#1}/{#2}}  % ma commande préférée
\newcommand{\nosqrt}[1]{{#1}^{\half}}  % également très pratique
\newcommand{\txts}{\textstyle}  % l'état de l'art en compression de formule
\newcommand{\eqsp}{\,}  % pour contrôler l'espace
\newcommand{\tb}{\textbullet\,}

% Parenthèses, Crochets et Accolades
\newcommand{\pr}[1]{\left({#1}\right)}
\newcommand{\prn}[1]{({\textstyle{#1}})}
\newcommand{\prbig}[1]{\big({#1}\big)}
\newcommand{\prBig}[1]{\Big({#1}\Big)}
\newcommand{\prbigg}[1]{\bigg({#1}\bigg)}
\newcommand{\prBigg}[1]{\Bigg({#1}\Bigg)}
\newcommand{\br}[1]{\left[{#1}\right]}
\newcommand{\bbr}[1]{\left\{{#1}\right\}}
\newcommand{\brn}[1]{[{\textstyle{#1}}]}
\newcommand{\brbig}[1]{\big[{#1}\big]}
\newcommand{\brBig}[1]{\Big[{#1}\Big]}
\newcommand{\brbigg}[1]{\bigg[{#1}\bigg]}
\newcommand{\ac}[1]{\left\{{#1}\right\}}
\newcommand{\acn}[1]{\{{\textstyle{#1}}\}}
\newcommand{\acbig}[1]{\big\{{#1}\big\}}
\newcommand{\acBig}[1]{\Big\{{#1}\Big\}}
\newcommand{\acbigg}[1]{\bigg\{{#1}\bigg\}}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\normn}[1]{\|{\textstyle{#1}}\|}
\newcommand{\ninf}[1]{\norm{#1}_\infty}
\newcommand{\abs}[1]{\left\lvert{#1}\right\rvert}
\newcommand{\absn}[1]{\lvert{#1}\rvert}
\newcommand{\ps}[2]{\left\langle{#1},{#2}\right\rangle}  % produit scalaire
\newcommand{\psn}[2]{\langle\textstyle{#1},{#2}\rangle}  % produit scalaire

% On définit les commandes sur les symbôles
\newcommand{\gauss}{\mathrm{N}}
% \newcommand{\loiGauss}{\gauss}
\newcommand{\wass}{W_{2}}
% \newcommand{\dwn}{\mathcal{C}_{dwn}}
\newcommand{\up}{\mathscr{C}}
\newcommand{\Adwn}{\mathcal{A}_{down}}
\newcommand{\Aup}{\mathcal{A}_{up}}
% \newcommand{\epsdwn}{\varepsilon^{(dwn)}}
% \newcommand{\epsup}{\varepsilon^{(up)}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\U}{U}
\newcommand{\M}{M}
\newcommand{\lip}{\mathtt{L}}
\newcommand{\barM}{\bar{\mathtt{M}}}
\newcommand{\MU}{M}
\newcommand{\mU}{\mathtt{m}}
\newcommand{\grad}{H}  % \textsl{H}
\newcommand{\tgrad}{\tilde{H}}
\newcommand{\tgradD}{F}

\newcommand{\qslds}{$\texttt{QLSD}^\star$}
\newcommand{\qsld}{{\texttt{QLSD}}}
\newcommand{\qsldpp}{$\texttt{QLSD}^{++}$}
\newcommand{\qlsds}{$\texttt{QLSD}^\star$}
\newcommand{\qlsdsharp}{$\texttt{QLSD}^{\#}$}
\newcommand{\qlsd}{{\texttt{QLSD}}}
\newcommand{\qlsdpp}{$\texttt{QLSD}^{++}$}
\def\Bs{\Btt^{\star}}
\def\tBs{\tilde{\Btt}^{\star}}
\def\sigmas{\sigma_{\star}}
\def\MH{\Mtt}
\def\tMH{\tMtt}
\def\thetas{\theta^{\star}}
\def\bMH{\bar{\MH}}
\def\Pens{\mathcal{P}}
\def\tkappa{\tilde{\kappa}}
\def\Dg{\mathrm{D}_{\gamma}}
\def\DgZ{\mathrm{D}_{0,\gamma}}
\def\wpN{\wp_N}
\def\card{\mathrm{card}}
\def\wpNn{\wp_{N,n}}
\def\Fs{F^{\star}}
\def\Hs{H^{\star}}
\def\balpha{\bar{\alpha}}


\makeatletter
\newcommand{\ostar}{\mathbin{\mathpalette\make@circled\star}}
\newcommand{\pstar}{\mathbin{\mathpalette\make@circled+}}
\newcommand{\make@circled}[2]{%
  \ooalign{$\m@th#1\smallbigcirc{#1}$\cr\hidewidth$\m@th#1#2$\hidewidth\cr}%
}
\newcommand{\smallbigcirc}[1]{%
  \vcenter{\hbox{\scalebox{0.77778}{$\m@th#1\bigcirc$}}}%
}
\makeatother
\def\ttheta{\tilde{\theta}}


==> section/tablefig/figure_align.tex <==

%
\begin{figure}
	~\hfill~\includegraphics[width=7.5cm]{../section/figs/align_iterations.png}~\hfill~ 
	\caption{Performance of \ours in function of the number of pretraining epochs of the feature
	transformation functions. The remaining hyperparameters of the training are similar to
those reported in the performance (\emph{e.g} we use $20$ epochs for training the PFL)}
	\label{fig:align}
\end{figure}

==> section/tablefig/figure_alparc.tex <==

%
\begin{figure}
		~\hfill~\includegraphics[width=4.cm]{./section/figs/align_iterations.png}~\hfill~ 
	~\hfill~\includegraphics[width=4.cm]{./section/figs/participation.png}~\hfill~ 
	%\caption{Performance of \ours with respects to the participation rate $r$.}
		\caption{Performance of \ours in function of (left) the number of pretraining epochs of the feature
		transformation functions, (right) the participation rate $r$.
		The remaining hyperparameters of the training are similar to
		those reported in the performance table (\emph{e.g} we use $20$ epochs for training the PFL).}
	\label{fig:alparc}
	\vspace{-0.5cm}
\end{figure}

==> section/tablefig/figure_toy.tex <==



==> section/theory.tex <==

\mv{Stopped here. To do: we have to provide theoretical insights that performing local learning of the reference measures followed by averaging in the Wasserstein space is equivalent to solving the Wasserstein barycenter problem, especially in the multiple local steps setting. This is similar to understanding the difference between gradient descent and FedAvg}


In this section, we provide some theoretical insights on the proposed methodology.
More precisely, we provide theoretical justification of the usage of the family of approximate distributions $\{\hat{\nu}_{\phi_i}^{(c)}; c \in \mathcal{Y}_i\}_{i \in [b]}$ in the Gaussian case.
In addition, we provide generalisation bounds showing the impact of the statistical heterogeneity across clients.
The proofs are postponed to the supplement.

\noindent \textbf{Justification of the usage of $\{\hat{\nu}_{\phi_i}^{(c)}\}$.}
In \eqref{eq:PFL_ERM_reg}, we are approximating the Wasserstein regularisation term by another one involving the family $\{\hat{\nu}_{\phi_i}\}$. 
In the following result, we provide theoretical support to this choice in the Gaussian scenario by showing that the random variable, defined as the error between these two Wasserstein terms, converges in distribution towards a zero-mean Gaussian random variable.


\noindent \textbf{Generalisation bound.}
The following result provides a generalisation bound on the risk associated to the $i$-th client with explicit dependencies on the discrepancy in the latent space $\Phi$ and heterogeneity in terms of number of observations.
\begin{theorem}
\label{theorem:2}
For any $i \in [b]$, let $\epsilon_i(g^{(i)}) = \mathbb{E}_{\phi_i(x) | y \sim \nu_{\phi_i}, y \sim p_i(y)}[\ell(g^{(i)}_{\theta_i}(\phi_i(x)),y)]$ the expected risk associated to the $i$-th client and $\hat{\epsilon}\pr{g^{(i)}} = \sum_{i=1}^b \sum_{j=1}^{n_i} \ell(g^{(i)}_{\theta_i}(\phi_i(x_i^{(j)})),y_i^{(j)})$ the empirical risk on data from all clients.
Let $n_i = |\mathrm{D}_i|$, $n=\sum_{i=1}^b n_i$ and $\delta \in (0,1)$.
Then, with probability at least $1-\delta$, we have 
    \begin{align}
        &\epsilon_i\pr{g^{(i)}} \leq \hat{\epsilon}\pr{g^{(i)}}  + \sqrt{\frac{4}{n}\pr{C \log\pr{\frac{2en}{C}}+ \log(4/\delta)}} \\
        &+ \sum_{j=1}^b \frac{n_j}{n}\mathrm{TV}\pr{\nu_{\phi_i},\nu_{\phi_j}}\eqsp, \label{eq:bound}
    \end{align}
where $C$ stands for the VC dimension of $\mathcal{G}$ so that $g^{(i)} \in \mathcal{G}$ and TV is the total variation distance.
\end{theorem}
In \eqref{eq:bound}, the first two terms are associated to the bound we would have obtained for a single client with the difference that the second term decreases as $1/n$ instead of $1/n_i$; showing how data from other clients could be leveraged to reduce the generalisation error.
The third term shows how discrepancy in the latent space impacts the expected risk of a single client.

\noindent \textbf{Impact of pretraining and connection with FedRep}.  
The algorithm we propose for personalized FL from heterogeneous data builds upon 
a core personalized FL algorithm which, in this case, is FedRep. We can show that, in some
extreme cases, the framework we propose boils down to some well-known situations. 
For instance, if we assume that each local transformation function
$\phi_i$ has been pretrained so that $\sum_{c \in \mathcal{Y}_i} \mathrm{W}_2^2 \pr{\mu_c,\nu_{\phi_i}^{(c)}} = 0 $, then data distributions on clients 
only differ by presence or absence of some classes. In such a case, the FL problem (with $\phi_i$ and $\nu$) can solved using a Federated (accelerated) stochastic gradient descent. Naturally, in practice, because we train $\phi_i$ only from samples, this situation is never attained. However, we can assume
that  for two pairs $(i,j)$ of clients the distance between $\nu_{\phi_i}^{(c)}$
and $\nu_{\phi_i}^{(c)}$ is small but non-zero. In this case, if we keep
the local transformation function fixed, then, from the latent space perspective, the FL problem boils down  to be the one solved by FedRep.




